Recurrent Early Exits for Federated Learning with Heterogeneous Clients

Federated learning (FL) has enabled distributed learning of a model across multiple clients in a privacy-preserving manner. One of the main challenges of FL is to accommodate clients with varying hardware capacities; clients have differing compute and memory requirements. To tackle this challenge, recent state-of-the-art approaches leverage the use of early exits. Nonetheless, these approaches fall short of mitigating the challenges of joint learning multiple exit classifiers, often relying on hand-picked heuristic solutions for knowledge distillation among classifiers and/or utilizing additional layers for weaker classifiers. In this work, instead of utilizing multiple classifiers, we propose a recurrent early exit approach named ReeFL that fuses features from different sub-models into a single shared classifier. Specifically, we use a transformer-based early-exit module shared among sub-models to i) better exploit multi-layer feature representations for task-specific prediction and ii) modulate the feature representation of the backbone model for subsequent predictions. We additionally present a per-client self-distillation approach where the best sub-model is automatically selected as the teacher of the other sub-models at each client. Our experiments on standard image and speech classification benchmarks across various emerging federated fine-tuning baselines demonstrate ReeFL's effectiveness over previous works.

==> icml2024/sections/3_backup.tex <==
\section{Proposed Method}


\subsection{Preliminaries}

%\textbf{Centralized Federated Learning.}~We consider a typical setting of FL where the central server holds the global weights $\theta_g$ which consists of $E$ early exits. Each client, $i$, has a device with a maximum resource budget of $r_i$ and $N_i$ private training examples denoted by $D_i := \{(\mathbf{x}_j, y_j)\}_{j=1}^{N_i}$ with $\mathbf{x}_j$ the input sample and $y_j$ the target label. For each round, $c$ participating clients are randomly sampled from a pool of $C$ clients and $\theta_g$ is split into sub-models to fit into each client's budget, $\theta_i = \theta_g[:r_i]$. These sub-models are then sent to the respective clients for training and the resulting trained models are sent back to the server and are aggregated depending on the aggregation strategy used, e.g. FedAvg~\cite{fedavg}, FedAdam~\cite{fedadam}, FedDyn~\cite{feddyn}. The resulting global model is then used in the next round. 

\textbf{Transformers with Early Exits.}~We primarily focus on the classical Transformers~\cite{vaswani2017attention, dosovitskiy2020image} due to their surge in popularity and also growing evidence of their capacity to better handle heterogeneous data in FL~\cite{qu2022rethinking}. A Transformer model typically consists of:
\begin{itemize}[leftmargin=*,noitemsep,topsep=0pt]
    \item A tokenizer that maps each element of the input sequence to a $d$-dimensional vector (aka token).
    \item A learnable positional embedding for each position $i$ is added to the outcome of tokenization, which gives the $i$-th token denoted by $z_i^0$.
    \item A learnable class token: $z_{\text{cls}}^0 \in \mathbb{R}^d$, where the superscript $0$ indicates it is located at the entrance.
    \item A stack of architecturally identical blocks that apply multi-head self-attention (MSA), layer normalization (LN) and feed-forward multilayer perceptron (MLP) transformations on the initial sequence of tokens $\mathbf{z}^0$. 
\end{itemize}
The forward pass of each Transformer block, for $l=1\cdots L$, takes the form:
{\small
\begin{align}
        &\mathbf{z}^l = \bar{\mathbf{z}} + \text{MLP}^l(\text{LN}_2^l(\bar{\mathbf{z}})) \notag \\
        &\bar{\mathbf{z}} = \mathbf{z}^{l-1} + \text{MSA}^l(\text{LN}_1^l(\mathbf{z}^{l-1})
        \label{eq:transformer}
\end{align}
}%
where $\mathbf{z}^l := [z_{\text{cls}}^l, z_1^l, \ldots, z_n^l]$ is the output from block $l$, yielding the $l$-th transformation of $\mathbf{z}^0$. Since none of the transformations change the shape of the intermediate representation $\mathbf{z}^l$, it can be fed into a classifier for early exiting.
% It becomes clear that none of the transformations change the shape of the intermediate representation $\mathbf{z}^l$, making it a potential early exit to the final (linear) classifier. To achieve scalability, the final classifier is shared among all early exits. 

\textbf{Federated Learning with Heterogeneous Clients.}~We consider a centralized setting of FL where the central server holds a global transformer model $\theta_g$ with sub-models $\theta_g[:l]$, for $l=1\cdots L$, representing $L$ early exits\footnote{One can reduce the number of sub-models by disabling some early exits. Each sub-model implies a certain budget.}. Each client, $i$, has a device with a maximum resource budget of $r_i$\footnote{This can signify computational, memory and/or bandwidth capabilities of the client.} and $N_i$ private training examples $\{(x_j, y_j)\}_{j=1}^{N_i}$ with $x_j$ the input sample and $y_j$ the target label. For each round, $c$ participating clients are randomly sampled from a pool of $C$ clients and the corresponding sub-models $\theta_i := \theta_g[:r_i]$ are selected to fit into each client's budget. These sub-models are then sent to the respective clients for training (i.e., one or few sub-model updating steps) and the updated sub-models are sent back to the server for central aggregation. Existing aggregation strategies such as FedAvg~\cite{fedavg}, FedAdam~\cite{fedadam}, FedDyn~\cite{feddyn} can be naturally adapted for the early-exit setting.
% , without affecting their convergence properties.


\subsection{Recurrent Early Exits}\label{sec:reefl}

As the class token/feature representation of earlier and deeper layers of the model differs, previous depth-based scaling FL works attached a classifier for each sub-model for early exiting. Each client then trains either the sub-model with the deepest classifier given its budget or trains all affordable sub-models, with the latter often outperforming the former as earlier classifiers are trained with more data~\cite{hong2022efficientsplitmix,kim2023depthfl}. Due to the conflicting gradients from different separate classifiers along with the imbalance in the data used to train different sub-models, existing works often use knowledge distillation, typically hand-picking the largest sub-model as the teacher~\cite{ilhan2023scalefl} or utilizing deep mutual learning~\cite{zhang2018deep} where each sub-model learned from one another~\cite{kim2023depthfl} to counteract these limitations.

\textbf{Architecture of \method{}.}~Unlike previous works, we propose to use a single classifier shared across all sub-models; the classifier is thus trained on the full dataset, overcoming the aforementioned problem where deeper classifiers underperform due to their being trained on a partial view of the dataset. In order to counteract the aforementioned limitation of handling diverse feature representations at different layers, we utilize a single-block Transformer, named \emph{\module{}}, which takes in a series of class tokens from the backbone Transformer model and learns to \textit{i)}~weight and fuse these class tokens for prediction and \textit{ii)}~build better feature representations from the backbone model. Specifically, in Fig~\ref{fig:overview}, \module{} takes in the class tokens at block $l$ as follows:
\begin{equation}
    % \begin{split}
    \mathbf{m}^l = \text{\module{}}_{\phi}([z_{\text{meta}}, z_{\text{cls}}^1, \ldots, z_{\text{cls}}^l] + \mathbf{p}), 
    % &z_{\text{cls}}^l \leftarrow m^l_{-1} \quad \text{with} \\
    % \end{split}
\end{equation}
where $\mathbf{m}^l := [m_0^l, \ldots, m_l^l]$ are the modulated class tokens, $\phi$ are the parameters of \module{}, $z_{\text{meta}}$ is the learnable meta-class token, 
%which is a representation of the backbone model's class tokens analogous to the class token in the backbone model, 
and $\mathbf{p}$ is the set of learnable positional embeddings.

Since We only 
The modulated meta-class token, $m^0$, is then used as an additive modification, adding discriminative features, to the current exit class token $z_{\text{cls}}^l$ as follows:
\begin{equation}
    \hat{y}^l =  \text{Classifier}_{\psi}(m^0 + z_{\text{cls}}^l)
\end{equation}
where $\psi$ are the parameters of the shared classifier.
After which, The modulated class token at block $l$, $m^{l}$, is then used to modulate the feature representations of the backbone model as follows:
\begin{equation}
\label{eq:mod_cls_token}
    z_{\text{cls}}^l \leftarrow m^l
\end{equation}
where $z_{\text{cls}}^l$ is used as an input to the next backbone block (Eq.~\ref{eq:transformer}). Note that the original class token $z_{\text{cls}}^l$ is first used for prediction before it is replaced with the modulated token. Hence, \module{} learns to concurrently \textit{ii)}~modulate the backbone class tokens for better feature learning and \textit{ii)}~exploit for task-based prediction by adding discriminative features to the respective exit's class token via the modulated meta-class token.

\textbf{Federated Training of \method{}.}~In each federated round, for each client, we train $\theta_i$ which consists of both $\phi$ and $\psi$ on the local train dataset using SGD. Note that in the case where the backbone model is frozen, then the learnable parameters of $\theta_i$ will be exactly $\phi$ and $\psi$. Following previous works~\cite{kim2023depthfl,ilhan2023scalefl}, each client, $i$, aims to minimize the following loss:
\begin{equation}
    \mathcal{L}_i = \sum_{e=1}^{E_{r_i}} \mathcal{L}_e^{ce} + \eta \mathcal{L}^{kl}
\end{equation}
where $E_{r_i}$ is the maximum exit within the client's budget, $\mathcal{L}_e^{ce}=\frac{1}{N_i}\sum^{N_i}_{j=1} \mathcal{L}^{ce}(\hat{y}^e_j,y_j)$ is the cross-entropy (CE) loss of the $e$-th exit, $\mathcal{L}^{kl}$ is the Kullback–Leibler (KL) loss denoting knowledge transfer between sub-models with its corresponding hyperparameter $\eta$. 
At the end of each round, participated clients send their locally trained parameters back to the server where these parameters will be aggregated using FedAvg~\cite{fedavg}. As the clients have different resource budgets, we weight the overlapping parameters accordingly to the number of data samples used to train each parameter. 
% Note that if there is an exit after every block, $E=L$. 

\textbf{\method{}'s Knowledge Distillation.}~In many prior works, the teacher and student sub-models in $\mathcal{L}^{kl}$ are manually defined, \textit{e.g.} from a bigger model to a smaller model~\cite{horvath2021fjord,ilhan2023scalefl} or the use of deep mutual learning~\cite{zhang2018deep} where all sub-models learn from one another~\cite{kim2023depthfl}. A major limitation of these approaches is that the teacher sub-model selected might be under-performing, especially in depth-scaling methods where the deepest sub-model is trained with partial data and the shallowest sub-model might not be sufficiently parameterized to learn good representations. The best-performing sub-model is hence dependent on the client, the model split, and the dataset on which it is optimized. Hence, instead of manually picking a teacher sub-model, \method{} uses the best training loss per-client to select the teacher sub-model and compute the KL loss as follows:
\begin{equation}    
    \mathcal{L}^{kl} = \frac{1}{N_i} \sum^{E_{r_i}}_{e \neq \tilde{e}} \sum^{N_i}_{j=1} (
    \sigma(\frac{\hat{y}_{j}^{\tilde{e}}}{\tau}) 
    \log \frac{\sigma(\frac{\hat{y}^{\tilde{e}}_j}{\tau})}                  {\sigma(\frac{\hat{y}_{j}^e}{\tau})}
    ) \tau^{2}
    % 
\end{equation}
where $\tilde{e} = \argmin \bar{\mathcal{L}^{ce}} = \argmin [\mathcal{L}_1^{ce}, \ldots, \mathcal{L}_{E_{r_i}}^{ce}]$ is the exit with the lowest training CE loss, $\sigma$ is the softmax function and $\tau$ is the temperature.
In practice, as the training loss per mini-batch of data is noisy, we take the running estimate of the training loss per client: $\bar{\mathcal{L}^{ce}} = (1 - \zeta) * \bar{\mathcal{L}^{ce}} + \zeta * \bar{\mathcal{L}^{ce}_{new}}$ where $\zeta$ is a hyperparameter and $\bar{\mathcal{L}^{ce}_{new}}$ is the training CE loss of all exits within budget computed on a new mini-batch of data.




==> icml2024/tables/main_result_all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h!t]
\caption{Mean and standard deviation (SD) of the mean performance of all exits across 3 runs and the mean communication cost per round for each approach.}

\label{tab:mainres_all}
\begin{scriptsize}
\resizebox{1.0\textwidth}{!}{\begin{minipage}{\textwidth}
\begin{center}
\begin{tabular}{|c|l|l|ccc|c|c|c|}
\hline
\multicolumn{1}{|l|}{\multirow{2}{*}{No. of Exits}} & \multicolumn{1}{c|}{\multirow{2}{*}{Finetuning}} & \multicolumn{1}{c|}{\multirow{2}{*}{Approach}} & \multicolumn{3}{c|}{CIFAR-100} & \multirow{2}{*}{FEMNIST} & \multirow{2}{*}{SpeechCmds} & Comm. \\ \cline{4-6}
\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\alpha$=1000} & \multicolumn{1}{c|}{$\alpha$=1.0} & $\alpha$=0.1 &  &  & Costs (MB) \\ \hline
\multirow{30}{*}{4} & \multirow{5}{*}{Full} & ExclusiveFL & \multicolumn{1}{c|}{67.29±0.06} & \multicolumn{1}{c|}{66.66±0.18} & 60.91±0.11 & 84.07±0.09 & 73.69±0.05 & 53.31\\
 &  & InclusiveFL & \multicolumn{1}{c|}{61.04±0.03} & \multicolumn{1}{c|}{60.92±0.26} & 54.97±0.41 & 84.3±0.05 & 77.87±1.0 & 52.33\\
 &  & ScaleFL & \multicolumn{1}{c|}{57.84±0.1} & \multicolumn{1}{c|}{56.83±0.06} & 48.35±0.05 & 82.56±0.09 & 71.96±0.09 & 34.91\\
 &  & DepthFL & \multicolumn{1}{c|}{57.52±0.4} & \multicolumn{1}{c|}{55.25±0.03} & 45.79±0.27 & 81.24±0.37 & 78.44±0.38 & 53.31\\
 &  & ReeFL (ours) & \multicolumn{1}{c|}{\textbf{76.42±0.12}} & \multicolumn{1}{c|}{\textbf{75.69±0.17}} & \textbf{72.58±0.33} & \textbf{86.13±0.08} & \textbf{84.47±0.26} & 53.98\\ \cline{2-9} 
 & \multirow{5}{*}{Frozen} & ExclusiveFL & \multicolumn{1}{c|}{48.02±0.03} & \multicolumn{1}{c|}{47.04±0.08} & 41.2±0.08 & 48.09±0.03 & 17.26±0.19 & 1.12 \\
 &  & InclusiveFL & \multicolumn{1}{c|}{53.99±0.03} & \multicolumn{1}{c|}{53.23±0.02} & 49.08±0.01 & 63.0±0.02 & 26.53±0.03 & 0.15 \\
 &  & ScaleFL & \multicolumn{1}{c|}{28.5±0.04} & \multicolumn{1}{c|}{27.9±0.01} & 25.18±0.04 & 28.51±0.03 & 10.8±0.1 & 0.89\\
 &  & DepthFL & \multicolumn{1}{c|}{51.27±0.01} & \multicolumn{1}{c|}{49.07±0.05} & 28.63±0.54 & 45.49±0.84 & 24.37±0.09 & 1.12\\
 &  & ReeFL (ours) & \multicolumn{1}{c|}{\textbf{67.52±0.1}} & \multicolumn{1}{c|}{\textbf{66.48±0.03}} & \textbf{61.36±0.12} & \textbf{82.33±0.04} & \textbf{66.09±0.08} & 1.79\\ \cline{2-9} 
 & \multirow{5}{*}{LoRA} & ExclusiveFL & \multicolumn{1}{c|}{67.46±0.03} & \multicolumn{1}{c|}{66.4±0.03} & 58.78±0.06 & 82.98±0.09 & 69.93±0.1 & 2.53\\
 &  & InclusiveFL & \multicolumn{1}{c|}{69.37±0.02} & \multicolumn{1}{c|}{69.03±0.07} & 63.55±0.13 & 83.76±0.09 & 76.79±0.1 & 1.56\\
 &  & ScaleFL & \multicolumn{1}{c|}{45.68±0.04} & \multicolumn{1}{c|}{44.6±0.07} & 37.02±0.02 & 70.69±0.02 & 43.04±0.2 & 2.00\\
 &  & DepthFL & \multicolumn{1}{c|}{71.56±0.29} & \multicolumn{1}{c|}{70.18±0.27} & 64.33±0.05 & 82.35±0.21 & 77.15±0.13 & 2.53\\
 &  & ReeFL (ours) & \multicolumn{1}{c|}{\textbf{73.9±0.03}} & \multicolumn{1}{c|}{\textbf{73.37±0.07}} & \textbf{69.29±0.1} & \textbf{84.69±0.03} & \textbf{79.91±0.08} & 3.20\\ \cline{2-9} 
 & \multirow{5}{*}{PA} & ExclusiveFL & \multicolumn{1}{c|}{67.42±0.13} & \multicolumn{1}{c|}{66.48±0.19} & 59.0±0.04 & 82.35±0.16 & 69.82±0.02 & 2.55\\
 &  & InclusiveFL & \multicolumn{1}{c|}{66.81±0.04} & \multicolumn{1}{c|}{66.57±0.11} & 61.2±0.31 & 83.12±0.0 & 76.47±0.08 & 1.58\\
 &  & ScaleFL & \multicolumn{1}{c|}{46.48±0.01} & \multicolumn{1}{c|}{45.16±0.06} & 38.02±0.08 & 72.83±0.04 & 43.53±0.24 & 2.01\\
 &  & DepthFL & \multicolumn{1}{c|}{72.01±0.05} & \multicolumn{1}{c|}{70.79±0.08} & 64.92±0.23 & 82.54±0.17 & 74.46±0.24 & 2.55\\
 &  & ReeFL (ours) & \multicolumn{1}{c|}{\textbf{72.33±0.08}} & \multicolumn{1}{c|}{\textbf{71.44±0.05}} & \textbf{66.92±0.04} & \textbf{84.2±0.04} & \textbf{78.51±0.34} & 3.22\\ \cline{2-9} 
 & \multirow{5}{*}{SA} & ExclusiveFL & \multicolumn{1}{c|}{68.2±0.02} & \multicolumn{1}{c|}{67.39±0.07} & 59.71±0.09 & 82.07±0.04 & 68.98±0.2 & 2.55\\
 &  & InclusiveFL & \multicolumn{1}{c|}{67.5±0.18} & \multicolumn{1}{c|}{67.01±0.14} & 61.88±0.27 & 82.57±0.11 & 75.01±0.15 & 1.58\\
 &  & ScaleFL & \multicolumn{1}{c|}{41.88±0.01} & \multicolumn{1}{c|}{40.48±0.01} & 33.6±0.15 & 58.51±0.03 & 26.62±0.03 & 2.01\\
 &  & DepthFL & \multicolumn{1}{c|}{\textbf{72.63±0.18}} & \multicolumn{1}{c|}{71.3±0.02} & 64.73±0.04 & 81.92±0.17 & 74.7±0.23 & 2.55\\
 &  & ReeFL (ours) & \multicolumn{1}{c|}{72.15±0.07} & \multicolumn{1}{c|}{\textbf{71.48±0.1}} & \textbf{66.52±0.25} & \textbf{84.07±0.09} & \textbf{78.39±0.25} & 3.22\\ \cline{2-9} 
 & \multirow{5}{*}{SSF} & ExclusiveFL & \multicolumn{1}{c|}{66.06±0.02} & \multicolumn{1}{c|}{65.29±0.01} & 57.94±0.04 & 79.27±0.07 & 57.03±0.46 &1.39\\
 &  & InclusiveFL & \multicolumn{1}{c|}{67.6±0.04} & \multicolumn{1}{c|}{67.35±0.02} & 62.23±0.1 & 82.11±0.02 & 71.43±0.04 & 0.40\\
 &  & ScaleFL & \multicolumn{1}{c|}{40.12±0.09} & \multicolumn{1}{c|}{39.3±0.04} & 33.4±0.06 & 52.68±0.06 & 27.01±0.14 & 1.10\\
 &  & DepthFL & \multicolumn{1}{c|}{45.61±0.03} & \multicolumn{1}{c|}{42.87±0.11} & 28.38±0.42 & 74.66±0.22 & 66.22±0.12 & 1.39\\
 &  & ReeFL (ours) & \multicolumn{1}{c|}{\textbf{70.12±0.07}} & \multicolumn{1}{c|}{\textbf{69.54±0.02}} & \textbf{64.77±0.11} & \textbf{83.42±0.04} & \textbf{73.6±0.04} & 2.04\\ \hline
\multirow{30}{*}{12} & \multirow{5}{*}{Full} & ExclusiveFL & \multicolumn{1}{c|}{39.47±0.48} & \multicolumn{1}{c|}{38.26±0.21} & 31.11±0.08 & 77.07±0.06 & 64.71±0.18 & 46.39\\
 &  & InclusiveFL & \multicolumn{1}{c|}{42.35±2.18} & \multicolumn{1}{c|}{44.05±0.13} & 33.42±0.43 & 80.33±0.01 & 70.93±0.25 & 45.57\\
 &  & ScaleFL & \multicolumn{1}{c|}{35.63±0.09} & \multicolumn{1}{c|}{34.29±1.33} & 23.41±0.17 & 74.68±0.05 & 61.57±0.25 & 26.40\\
 &  & DepthFL & \multicolumn{1}{c|}{46.66±0.05} & \multicolumn{1}{c|}{43.6±0.52} & 33.69±0.4 & 78.34±0.23 & 71.23±0.34 & 46.39\\
 &  & ReeFL (ours) & \multicolumn{1}{c|}{\textbf{66.83±0.24}} & \multicolumn{1}{c|}{\textbf{65.89±0.19}} & \textbf{57.55±0.78} & \textbf{82.98±0.03} & \textbf{82.34±0.27} & 47.21 \\ \cline{2-9} 
 & \multirow{5}{*}{Frozen} & ExclusiveFL & \multicolumn{1}{c|}{39.19±0.01} & \multicolumn{1}{c|}{37.6±0.02} & 28.95±0.02 & 42.1±0.12 & 14.75±0.06 & 0.97\\
 &  & InclusiveFL & \multicolumn{1}{c|}{43.53±0.03} & \multicolumn{1}{c|}{41.6±0.04} & 32.28±0.05 & 53.35±0.03 & 20.22±0.05 & 0.15\\
 &  & ScaleFL & \multicolumn{1}{c|}{16.66±0.02} & \multicolumn{1}{c|}{15.4±0.01} & 11.77±0.01 & 20.98±0.05 & 7.32±0.1 & 0.70\\
 &  & DepthFL & \multicolumn{1}{c|}{45.22±0.06} & \multicolumn{1}{c|}{42.93±0.18} & 25.2±1.89 & 41.29±0.1 & 21.3±0.02 & 0.97\\
 &  & ReeFL (ours) & \multicolumn{1}{c|}{\textbf{58.74±0.05}} & \multicolumn{1}{c|}{\textbf{58.1±0.09}} & \textbf{51.33±0.36} & \textbf{75.36±0.02} & \textbf{59.5±0.5} & 1.79\\ \cline{2-9} 
 & \multirow{5}{*}{LoRA} & ExclusiveFL & \multicolumn{1}{c|}{48.04±0.05} & \multicolumn{1}{c|}{46.22±0.13} & 36.34±0.18 & 74.9±0.11 & 59.1±0.08 & 2.19\\
 &  & InclusiveFL & \multicolumn{1}{c|}{55.9±0.08} & \multicolumn{1}{c|}{54.54±0.15} & 41.53±0.15 & 78.21±0.15 & 66.18±0.58 & 1.37\\
 &  & ScaleFL & \multicolumn{1}{c|}{35.14±0.09} & \multicolumn{1}{c|}{33.05±0.02} & 22.62±0.1 & 59.57±0.05 & 44.23±0.14 & 1.58\\
 &  & DepthFL & \multicolumn{1}{c|}{62.74±0.09} & \multicolumn{1}{c|}{61.3±0.11} & 51.9±0.15 & 78.97±0.15 & 70.66±0.07 & 2.19\\
 &  & ReeFL (ours) & \multicolumn{1}{c|}{\textbf{65.7±0.09}} & \multicolumn{1}{c|}{\textbf{65.01±0.03}} & \textbf{58.85±0.05} & \textbf{81.06±0.06} & \textbf{75.96±0.18} & 3.01\\ \cline{2-9} 
 & \multirow{5}{*}{PA} & ExclusiveFL & \multicolumn{1}{c|}{45.63±0.14} & \multicolumn{1}{c|}{43.57±0.27} & 32.94±2.19 & 73.1±0.02 & 59.06±0.12 & 2.21\\
 &  & InclusiveFL & \multicolumn{1}{c|}{52.27±0.12} & \multicolumn{1}{c|}{50.97±0.06} & 39.41±0.03 & 73.04±0.03 & 63.05±0.23 & 1.39\\
 &  & ScaleFL & \multicolumn{1}{c|}{33.38±0.1} & \multicolumn{1}{c|}{31.48±0.04} & 21.72±0.22 & 62.0±0.05 & 44.08±0.07 & 1.60\\
 &  & DepthFL & \multicolumn{1}{c|}{61.23±0.23} & \multicolumn{1}{c|}{59.8±0.07} & 6.88±5.88 & 4.95±0.2 & 65.69±0.41 & 2.21\\
 &  & ReeFL (ours) & \multicolumn{1}{c|}{\textbf{62.35±0.07}} & \multicolumn{1}{c|}{\textbf{61.47±0.12}} & \textbf{55.67±0.14} & \textbf{77.62±0.04} & \textbf{72.37±0.02} & 3.03\\ \cline{2-9} 
 & \multirow{5}{*}{SA} & ExclusiveFL & \multicolumn{1}{c|}{47.69±0.04} & \multicolumn{1}{c|}{46.18±0.19} & 31.54±0.53 & 73.06±0.05 & 58.93±0.13 & 2.21\\
 &  & InclusiveFL & \multicolumn{1}{c|}{53.37±0.11} & \multicolumn{1}{c|}{52.02±0.06} & 40.06±0.1 & 72.54±0.07 & 61.8±0.19 & 1.39\\
 &  & ScaleFL & \multicolumn{1}{c|}{31.33±0.07} & \multicolumn{1}{c|}{28.97±0.05} & 19.27±0.02 & 53.08±0.01 & 31.65±0.11 & 1.60\\
 &  & DepthFL & \multicolumn{1}{c|}{62.66±0.09} & \multicolumn{1}{c|}{60.79±0.11} & 1.02±0.01 & 4.82±0.27 & 65.68±0.59 & 2.21\\
 &  & ReeFL (ours) & \multicolumn{1}{c|}{\textbf{63.28±0.13}} & \multicolumn{1}{c|}{\textbf{61.94±0.2}} & \textbf{54.99±0.1} & \textbf{77.43±0.04} & \textbf{71.52±0.13} & 3.03\\ \cline{2-9} 
 & \multirow{5}{*}{SSF} & ExclusiveFL & \multicolumn{1}{c|}{49.09±0.02} & \multicolumn{1}{c|}{47.69±0.08} & 18.66±1.7 & 69.43±0.03 & 54.94±0.22 &1.21\\
 &  & InclusiveFL & \multicolumn{1}{c|}{54.43±0.04} & \multicolumn{1}{c|}{52.92±0.07} & 40.63±0.01 & 74.48±0.02 & 59.6±0.09 & 0.37\\
 &  & ScaleFL & \multicolumn{1}{c|}{30.01±0.01} & \multicolumn{1}{c|}{27.99±0.05} & 19.24±0.03 & 46.63±0.02 & 25.17±0.12 & 0.87\\
 &  & DepthFL & \multicolumn{1}{c|}{47.31±0.2} & \multicolumn{1}{c|}{44.01±0.14} & 1.82±0.71 & 5.01±0.19 & 3.72±0.44 & 1.21\\
 &  & ReeFL (ours) & \multicolumn{1}{c|}{\textbf{61.85±0.02}} & \multicolumn{1}{c|}{\textbf{61.25±0.17}} & \textbf{54.42±0.13} & \textbf{78.05±0.03} & \textbf{67.44±0.24} & 2.01\\ \hline
\end{tabular}
\end{center}
\end{minipage}
}
\end{scriptsize}
\end{table*}
